FlexCloud: Direct, Modular Georeferencing and Drift-Correction of Point Cloud Maps

Current software stacks for real-world applications of autonomous driving leverage map information to ensure reliable localization, path planning, and motion prediction. An important field of research is the generation of point cloud maps, referring to the topic of simultaneous localization and mapping (SLAM). As most recent developments do not include global position data, the resulting point cloud maps suffer from internal distortion and missing georeferencing, preventing their use for map-based localization approaches. Therefore, we propose FlexCloud for an automatic georeferencing of point cloud maps created from SLAM. Our approach is designed to work modularly with different SLAM methods, utilizing only the generated local point cloud map and its odometry. Using the corresponding GNSS positions enables direct georeferencing without additional control points. By leveraging a 3D rubber-sheet transformation, we can correct distortions within the map caused by long-term drift while maintaining its structure. Our approach enables the creation of consistent, globally referenced point cloud maps from data collected by a mobile mapping system (MMS). The source code of our work is available at https://github.com/TUMFTM/FlexCloud.

==> fig/data/yas_cp_10cp.tex <==
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (29.8166, -112.314, 33.5799) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (195.573, 169.306, 39.1297) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (52.0361, 549.037, 37.702) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-88.0065, 691.426, 34.8659) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-239.539, 235.367, 36.0502) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-390.313, -220.308, 34.1356) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-148.464, -580.092, 34.5874) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (253.31, -841.714, 34.6342) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (169.703, -702.293, 33.727) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-275.91, -254.703, 34.8609) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-484.144, -1035.19, -280.446) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-485.06, 1008.29, -274.063) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (488.84, 1006.28, -279.469) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (488.828, -1037.1, -272.534) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-484.144, -1035.19, 357.169) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (-485.06, 1008.29, 363.552) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (488.84, 1006.28, 358.147) };
        \addplot3[only marks, mark=asterisk, color=TUMAccentOrange] coordinates { (488.828, -1037.1, 365.081) };


==> fig/data/yas_triag_10cp.tex <==
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (-277.077, -254.12, 36.0033) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-277.077, -254.12, 36.0033) (-148.504, -581.19, 33.0633) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-148.504, -581.19, 33.0633) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, -281.97) (-484.183, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, -281.97) (-391.226, -220.922, 31.586) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-391.226, -220.922, 31.586) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (-484.183, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-239.135, 234.391, 37.5893) (30.1911, -112.815, 43.2818) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (30.1911, -112.815, 43.2818) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (-239.135, 234.391, 37.5893) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (-484.183, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (-484.183, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, 1007.16, 355.645) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (-87.13, 690.288, 26.9592) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-87.13, 690.288, 26.9592) (53.0294, 549.916, 35.2006) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (53.0294, 549.916, 35.2006) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (489.833, 1007.16, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, 355.645) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, 1007.16, -281.97) (195.768, 169.439, 49.3182) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (195.768, 169.439, 49.3182) (489.833, -1036.29, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, -281.97) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (489.833, 1007.16, -281.97) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (-484.183, -1036.29, 355.645) (254.315, -840.901, 25.198) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (254.315, -840.901, 25.198) (169.05, -701.569, 31.8336) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (169.05, -701.569, 31.8336) (489.833, -1036.29, 355.645) };
        \addplot3[color=TUMAccentGreen, thin] coordinates { (489.833, -1036.29, 355.645) (-484.183, -1036.29, 355.645) };

